Interpretable machine learning for high-dimensional trajectories of aging health

We have built a computational model for individual aging trajectories of health and survival, which contains physical, functional, and biological variables, and is conditioned on demographic, lifestyle, and medical background information. We combine techniques of modern machine learning with an interpretable interaction network, where health variables are coupled by explicit pair-wise interactions within a stochastic dynamical system. Our dynamic joint interpretable network (DJIN) model is scalable to large longitudinal data sets, is predictive of individual high-dimensional health trajectories and survival from baseline health states, and infers an interpretable network of directed interactions between the health variables. The network identifies plausible physiological connections between health variables as well as clusters of strongly connected health variables. We use English Longitudinal Study of Aging (ELSA) data to train our model and show that it performs better than multiple dedicated linear models for health outcomes and survival. We compare our model with flexible lower-dimensional latent-space models to explore the dimensionality required to accurately model aging health outcomes. Our DJIN model can be used to generate synthetic individuals that age realistically, to impute missing data, and to simulate future aging outcomes given arbitrary initial health states.

==> OLD/cutouts.tex <==
% CUTOUT

 %In .~\ref{Synthetic classification}B, we see that the classification accuracy is relatively constant for different numbers of observed variables, but thewhen there are many observed deficits, the classifier can better distinguish between the populations -- note however that the ratio does not exceed 0.6. Furthermore, in Fig.~\ref{Synthetic classification}C, we show that the number of individuals with large numbers of observed deficits is small. This a limitation of the dataset, where we are not able to train the model on many individuals with mostly observed deficits.
 
%While our DJIN model outperforms regularized linear models quantitatively, it is also attractive qualitatively. As a joint model, our model includes an estimate of absolute risk of death as individuals age with the survival function. Health variables are modeled with dynamics coupled together through a causal interaction network, rather than a constant slope determined at baseline as in the linear models. This leads to health variable trajectories continually interacting with feedback as an individual ages.  

%\includegraphics[width=0.32\textwidth]{Generated_population_mean_job_id12_nf.pdf}
%\includegraphics[width=0.32\textwidth]{Aggregated_population_mean_job_id12_nf.pdf}
%{\bf G)} Generated population mean and observed population mean for 5-year age bins from ages 65 to 85 for the z-scores of all health variables. The dashed line shows the exact result. {\bf H)} Aggregate mean of all the z-scores for each health variable vs age for the generated synthetic population (blue) and the observed test population (red). The filled regions shows the standard deviations.     

%Estimating an individual's ``Biological Age'' is a common approach, typically with DNA methylation markers \cite{Hannum:2013, Horvath:2013, Levine:2018, Lu:2019, Li:2020}, but also the plasma proteome \cite{Lehallier2019} and gut microbiome \cite{Galkin:2020}. Simpler clinical summary measures also exist \cite{Mitnitski:2001, Fried:2001}.

%Nevertheless, these measures only summarize the progression of aging into a single dimension, and cannot capture the full high-dimensionality of aging trajectories. Additionally, these summaries cannot be used for individualized predictions of future health outcomes, and can only indicate an increased risk of aging-related diseases. Approaching these problem requires predictive models of these high-dimensional trajectories, and we introduce a novel model to approach to this problem.

in a more general approach than is typically done with biological age. %These models all operate in different scenarios for time-series data, survival data, ..
%Joint models for longitudinal and survival data include both health and mortality to model individual trajectories , although these models are typically focused on modeling outcomes for specific diseases from longitudinally measured health variables as input. 

%While these initial studies have used the high-dimensional data for predictive measurements, they have not predicted the high-dimensional trajectories themselves.
%Avchaciov \emph{et al}. \cite{Avchaciov:2020} infer a 1-dimensional dynamic summary measure of aging in mice that correlates with mortality and treatment effects, but did not consider modelling mortality or predictions of future health.
%In one such study, Pierson \emph{et al}. \cite{Pierson:2019} use cross-sectional data to learn interpretable ``rates of aging'' for each individual that correlate with common risk factors of aging, and can be used to forecast aging trajectories. However they did not consider mortality

%  The multiple scales available in this data, including both physical assessments of functional abilities and biological measurements like blood/urine chemistry and omics, raises the question of how to use this data to develop a unifying model of aging that integrates the many scales involved in aging and provides an understanding of how damage at the biological level propagates to damage at the functional level \cite{Ferrucci:2018, Mitnitski:2019}. In this work we focus on building a predictive and interpretable model of high-dimensional aging trajectories. 

The health variables in the dataset include blood biomarkers, physical/function measures typical in a clinical frailty assessment, and survey questions about general health and lifestyle. 

-- while using less structured techniques
We build our assumption of aging as network of interacting components into our model, while learning unknown components with complex neural networks. This approach has been branded 
 We use stochastic differential equations (SDEs) to model the stochastic evolution of an individual's health state with age, and the corresponding mortality rate describing the evolution of their survival probability. In these SDEs, we model pairwise interactions between health variables with a network, while parameterizing other unknown components with neural networks. The explicit interaction network adds interpretability, despite the complexity of components of the model. To deal with missing data, we include a component of the model to impute the baseline health state. 
 
 
%Our model predicts longitudinal forecasts of future health trajectories and survival probability. Our model is robust to noisy data, missing data, mortality censoring, and non-uniform follow-up times. Additionally, our model infers an interpretable interaction network describing the effective strength of interactions between health variables from the longitudinal data. This shows that our model is not just making ``black-box'' predictions, and highlights some of the realistic physiological connections used in these predictions.

%We use variational Bayesian inference for SDEs \cite{Archambeau:2007, Opper:2019} and Neural SDEs \cite{LiDuvenaud:2020} to approximate the posterior distribution of the health and survival trajectories, network weights, measurement error, and imputed missing values, 
%\begin{align}
%    & p(\mathcal{T}, \mathbf{w}, \mathbf{\sigma_y}, \mathbf{\sigma_x},\bm{\theta}, \mathbf{x}_0, \mathbf{z}|\{\mathbf{y}_{t_i}\}_i,\mathbf{u}_{t_0}, \mathbf{o}_{t_0})) .
%\end{align}

so that within the bin $[p, p+\epsilon]$ of the survival curves, we would expect $\epsilon\%$ of the individuals to live longer than the age for which this probability occurs.


%Spearman's rank correlation scores are denoted by $\rho$ for the comparison of the rank-ordering of the RMSE scores for each variable, relative to the $3$ year scores. The ordering stays relatively similar, indicating that it is generally the same variables that are predicted well or poorly.

We use a strict criteria for the existence of a connection --- whether the 99\% credible interval of the posterior is fully above or below zero. This criteria is seen in supplemental Fig.~\ref{network inference}C). This also shows that the all uncertain connections are centered around zero weight. % move to supplemental



%We specifically build our model to take into account some of the difficulties of using large cohort data for aging. 

\section{Related models}

Our model is similar to stochastic process joint models of aging developed and used by Anatoliy Yashin and collaborators \cite{Yashin:2007, Arbeev:2011, Yashin:2012, Arbeev:2014, Zhbannikov:2017}. These models also represent the dynamics of individual health variables with stochastic differential equations, and compute mortality rates and survival probability from these health trajectories. However, this model has not been scaled up and applied with many health variables or large longitudinal data-sets. 

The details of our model uses ideas from Neural SDE models \cite{Tzen:2019, LiDuvenaud:2020} and variational Bayesian inference for SDEs \cite{Archambeau:2007, Opper:2019}. We use the same method of approximating the posterior distribution for the trajectories with an SDE with a neural network for the arbitrary drift function. The main differences here are the use of strong assumptions on the prior SDE to add interpretability to the model, and the mortality rate included for modeling survival. In addition, our dynamics occur directly on the (imputed) observed variables rather than inferred latent variables, so that we can infer an interaction network describing the dynamics of these observed variables.

We take a variational Bayesian approach similar to Ryder \emph{et al.} \cite{Ryder:2018}, computing an approximate posterior for the trajectories and parameters of an SDE. However, they use a discrete-time approach to computing the posterior of the trajectories, instead of a continuous-time SDE as used here.

Joint longitudinal-survival models typically take a longitudinally-tracked input and fit a model to  these for the trajectories of observed health outcomes \cite{Henderson:2000}. Usually these are used to adjust inferences for informed dropout in the statistical analysis of longitudinal studies or improve models of survival outcomes by including time-varying inputs \cite{Hickey:2016}. Although joint longitudinal-survival models focused on prediction of health outcomes do exist \cite{Lim:2018}. Our approach is distinct....



\subsection{Variational inference for SDEs}
\emph{2. SDE trajectories}

Given a simulated stochastic trajectory and survival function $\mathcal{T} = (\{\mathbf{x}(t)|\mathbf{t}_{t_0},\mathbf{u}_{t_0}\}_t,\,\{S(t)|\mathbf{t}_{t_0},\mathbf{u}_{t_0}\}_t$) sampled from the model for an individual $m$ with baseline variables $\mathbf{x}(t_0)$, we compute a conditional likelihood,
%
\begin{gather} \label{conditional likelihood}
    \log{p(\mathcal{D}|\mathcal{T},\mathbf{\Sigma_y}})
    = \\ \nonumber \sum_m\Big(c^{(m)}\log{S(a^{(m)})} + (1-c^{(m)})\big[\log{\Gamma(a^{(m)})} \\  \nonumber + \log{S(a^{(m)})}\big]\Big) \\ \nonumber
    + \sum_{m,k,i}o_{t_k, i}^{(m)}\log{\mathcal{N}\big(\psi_i(y_{t_k,i}^{(m)})|x_i(t_k^{(m)}), \Sigma_{y,ii}\big)}.
\end{gather}
%
This contains the censored and uncensored likelihood for survival, and the Gaussian likelihood for health variables. Unobserved health variables are masked by observation mask $\mathbf{o}_{t_k}$. 

Using Bayes theorem, the posterior can be expressed as,
\begin{eqnarray} \nonumber
    p(\mathcal{T}, \mathbf{w},\mathbf{\sigma_y}|\mathcal{D}) = \frac{ p(\mathcal{D}|\mathcal{T}, \mathbf{\sigma_y}) p(\mathcal{T}|\mathbf{w},\bm{\theta}) p(\mathbf{w})p(\mathbf{\sigma_y})}{p(\mathcal{D})}.
\end{eqnarray}
In this formulation, we take the dynamics in Eqn.~\ref{dynamics} and \ref{survival} as defining a prior SDE, which generates sample from the prior distribution of the trajectories $p(\mathcal{T}|\mathbf{w},\theta)$. The prior for the network weights is $p(\mathbf{w})$ and the prior for the measurement error is $p(\mathbf{\sigma_y})$. 

We use an approximate variational Bayesian approach to infer the posterior distribution of the trajectories and parameters \cite{Ryder:2018, Opper:2019, LiDuvenaud:2020}. We make a factorized variational approximation for the posterior $p(\mathcal{T},\mathbf{w}|\mathcal{D}, \theta)$,
\begin{eqnarray}
    q(\mathcal{T}, \mathbf{w},\mathbf{\sigma_y}|\phi) = q(\mathcal{T}| \phi_\mathcal{T})q(\mathbf{w}|\phi_\mathbf{w})q(\mathbf{\sigma_y}|\phi_\mathbf{\sigma}),
\end{eqnarray}
where we denote the new variational parameters to be learned by $\phi$. In this approximation we learn a new SDE that generates samples from the approximate posterior for the trajectories $q(\mathcal{T}|\phi_\mathcal{T})$. This SDE has the same diffusive noise, but modified drift (this restriction on the noise is fully general, \cite{Opper:2019}),
\begin{eqnarray} \label{posterior}
    \dot{\mathbf{x}}(t) = g(\mathbf{x}, \mathbf{v}, t;\phi) + \epsilon_x. 
\end{eqnarray}
We use a Laplace distribution as a shrinkage prior for the network connection weights and Gamma distribution for the measurement error prior, and similarily use distinct independent Laplace distributions for the approximate posterior of every network connection,



The parameters and variational parameters $(\theta, \phi)$ are optimized together by maximizing a standard lower bound \cite{Blei:2017},
\begin{eqnarray} \nonumber
    \log{p(\mathcal{D})} &\geq& \\ \nonumber
    && \mathbb{E}_{\mathcal{T}, \mathbf{w},\mathbf{\sigma_y} \sim q}\Big[\log{p(\mathcal{D},\mathcal{T},\mathbf{w},\mathbf{\sigma_y})} - \log{q(\mathcal{T},\mathbf{w},\mathbf{\sigma_y}|\phi)}\Big]. 
\end{eqnarray}

As derived by others \cite{Archambeau:2007, Opper:2019}, this takes the following form for SDEs,

\begin{eqnarray} \nonumber
    \log{&&p(\mathcal{D}|\theta)} \geq \sum_m\mathbb{E}_{\mathcal{T},\mathbf{w}\sim q}\Bigg[\sum_{k}\log{\mathcal{N}\big(\bm{\psi}(\mathbf{y}_{t_k}^{(m)})|\mathbf{x}(t_k^{(m)}), \mathbf{\Sigma}_y\big)} \\ \nonumber &&+ c^{(m)}\log{S(a^{(m)})} + (1-c^{(m)})\big[\log{\Gamma(a^{(m)})} + \log{S(a^{(m)})}\big] \\ \nonumber
    && - \frac{1}{2}\int_{t_0^{(m)}}^{a^{(m)}}\Big|\Big|\mathbf{\Sigma}_x^{-1/2}\big(\mathbf{\mu}(\mathbf{x}, \mathbf{v}, t;\theta, \mathbf{w}) - \mathbf{g}(\mathbf{x}, \mathbf{v}, t;\phi)\big)\Big|\Big|^2dt \Bigg] \\ \nonumber
    &&- KL(q(\mathbf{w}|\phi_w)||p(\mathbf{w})), \label{ELBO}
\end{eqnarray}


%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% CUTOUTS


%This can be reformulated as linear regression. Define:
%\begin{eqnarray} \nonumber
%\Delta y_{k,i}^{(m)} &\equiv& y_{t_k,i}^{(m)} - y_{t_0,i}^{(m)} \\ \nonumber
%\tilde{\mathbf{y}}_{k,i}^{(m)} &\equiv& \mathbf{y}_{t_0}^{(m)} (t_{k,i}^{(m)} - t_{0,i}^{(m)}) \\ \nonumber
%\tilde{\mathbf{u}}_{k,i}^{(m)} &\equiv& \mathbf{u}_{t_0}^{(m)} (t_{k,i}^{(m)} - t_{0,i}^{(m)}) \\ \nonumber
%\tilde{t}_{k,i} &\equiv& t_{0,i}^{(m)}(t_{k,i}^{(m)} - t_{0,i}^{(m)})
%\end{eqnarray}

%Then we can formulate this model as linear regression:
%\begin{eqnarray}
%\Delta y_{k,i}^{(m)} &=& \beta_{0,i}\tilde{t}_{k,i}^{(m)} + \bm{\beta}_{1,i}\cdot \tilde{\mathbf{y}}_{k,i}^{(m)} + \bm{\beta}_{1,i}\cdot \tilde{\mathbf{u}}_{k,i}^{(m)} \nonumber
%\end{eqnarray}
%We fit this model with elastic net regression for the coefficients.


%We train our model with the English Longitudinal study of Aging (ELSA \cite{ELSA}). We combine all 8 waves of ELSA, to get data for $25290$ individuals. We extract and use $29$ health variables, which include a wide variety of physical/functional and molecular variables, in addition to $19$ relevant background variables. In Supplemental Fig.~\ref{ELSA data}, we list all variables used, and the number of individuals for which the variable is available at different times from baseline.

%At each observation time, not all health variables are observed. This is due to different scheduled times for certain variables (i.e. those requiring specific laboratory tests) and missing values (both random and due to health complications). This means the times $t_k$ are not uniformly spaced, and there are different intervals of measurement for different variables. Individual survival is also often censored: for uncensored individuals we have a reported death age, for censored individuals we only have last age known alive.

%\subsection{Network models}
%Farrell \emph{et al} \cite{Farrell:2020} developed a network model of aging to generate synthetic health trajectories and predict survival. In this model, nodes represent health variables that can damage stochastic rates. The damage rate of a node is determined by a weighted sum,
%\begin{eqnarray}
%f_i &=& \sum_{j=1}^N w_{ij}x_i + \mu_i(t) \\
%\Gamma_i &=& \sum_{n=0}^3 \gamma_nf_i^n
%\end{eqnarray}

%\subsection{Stochastic process joint models}
%Anatoliy Yashin and collaborators developed stochastic process joint models of aging \cite{Yashin:2007, Arbeev:2011, Yashin:2012, Arbeev:2014}. These models represent the dynamics of an individuals health state $\mathbf{y}(t)$ with a stochastic differential equation, 
%
%\begin{eqnarray}
%\dot{\mathbf{y}}(t) = \mathbf{A}(t, \mathbf{u})(\mathbf{y}(t) - \mathbf{f}_1(t, \mathbf{u})) + \mathbf{B}(t, \mathbf{u})\mathbf{\epsilon}_y(t),\,\,\mathbf{\epsilon}_y\sim\mathcal{N}(0,\mathbf{I})
%\end{eqnarray}
%
%and model survival with a mortality rate $\Gamma(\mathbf{y}, t)$ that is marginalized \cite{Yashin:1997} to determine a survival function of the usual form for survival models, 
%
%\begin{eqnarray} \label{exponential survival}
%  S(t|\mathbf{y}, \mathbf{u}) = \exp{\big(-\int_0^t \bar{\Gamma}(\tau)d\tau\big)}. 
%\end{eqnarray}

%This model was used with synthetic data or small-sized observational data with one or two variables, but has never been  applied to large and high dimensional datasets for individual aging trajectories. Our approach builds upon these models, with many modifications to improve the model and deal with the difficulties of  longitudinal aging studies with high-dimensional data.
% extol both the promise of these models and the challenge, which we meet


%The reconstruction likelihood for the auto-encoder is in the $n = 0$ term of this sum. The likelihood terms for mortality are the survival function $S(t_c^{(m)}|\mathbf{x}, \mathbf{u})$ for censored individuals and the death age probability $p(t_d^{(m)}|\mathbf{x}, \mathbf{u}) = -\dot{S}(t_d^{(m)}|\mathbf{x}, \mathbf{u})$ for uncensored individuals. The observation likelihood is computed, 
%
%\begin{eqnarray} \nonumber
%\log{p(\{Y^{(m)}\}, \{a^{(m)}\}|\mathbf{x}(t),\theta)} &=& \sum_{m,n,i} \Big[-\frac{1}{2}\log{(2\pi\mathbf{\Sigma}_{y,ii})} -\frac{1}{2\mathbf{\Sigma}_{y,ii}}m_{t_0, i}^{(m)}\big(y^{(m)}_{t_n,i} - x_i(%t_n)\big)^2\Big] \\ &+&  \sum_{m}(1-c^{(m)})\big[\log{\Gamma(\mathbf{x},\mathbf{u}^{(m)}, t_d^{(m)})} + \log{S(t_d^{(m)}|\mathbf{x}, \mathbf{u}^{(m)})}\big] \nonumber \\ 
%&+& \frac{1}{\mathbb{S}}\sum_{s,m}c^{(m)}\log{S(t_c^{(m)}|\mathbf{x}, \mathbf{u}^{(m)})}, 
%\end{eqnarray} %+ \frac{1}{2}\sum_i\Big[1 + \log{\big(\frac{\Sigma_{y,ii}}{\sigma_{y0}^2}\big)} - \frac{\Sigma_{y,ii}}{\sigma_{y0}^2}\Big]


%\cite{Tsiatsias, Henderson:2000, Brown:2003, Hickey:2016}
%\begin{eqnarray}
%\mathbf{y}_{t_n} &=& \mathbf{x}(t_n) + \epsilon(t_n) \\
%\mathbf{x}(t) &=& \mathbf{x}(t_0) + \mathbf{b}(\mathbf{x}(t_0), \mathbf{u}, t_0)(t - t_0) %\\
%\mathbf{b}(\mathbf{x}(t_0), \mathbf{u}, t_0) &=& \mathbf{W}_{x}\mathbf{x}(t_0) + %\mathbf{W}_{u}\mathbf{u} + \mathbf{w}_{t}t_0.
%\end{eqnarray}
%The sex and age-dependent training-set population mean is used for initially missing values at age $t_0$.

%For the survival component, we use a standard Cox-proportional hazards model with a ``current value'' association structure \cite{Hickey:2016},

%\begin{eqnarray}
%\lambda(t) &=& \lambda_0(t)\exp{\Big(\gamma_0 + %\bm{\gamma}_x\cdot\mathbf{x}(t) + \bm{\gamma}_u\cdot\mathbf{u} %\Big)} \\
%\lambda_0(t) &=& \exp{\Big(\lambda_{00} + \lambda_{01}t + %\lambda_{02}t^2\Big)} \\
%S(t) &=& \exp{\big(-\int_0^t\lambda(t')dt'\big)}.
%\end{eqnarray}


%where $s^{(m)}$ are individual sample weights as described in Appendix section \ref{augmentation}.

%\begin{figure}[h] 
%    \includegraphics[width=\textwidth]{Test_Longitudinal_values_3years_job_id0.pdf}
%    \caption{}
%    \label{predicted vs exact}
%\end{figure}


%\begin{figure}[h] 
%    %\includegraphics[width=\textwidth]{Network_Test_id15.pdf}
%    \includegraphics[width=\textwidth]{Test_plot_context_sex_TSNE_job_id47.pdf}
%    \caption{Visualizing $\mathbf{v}$ with t-SNE.}
%    \label{context}
%\end{figure}
%In Fig.~\ref{context} we use t-SNE \cite{tsne} to visualize the individual-specific information $\mathbf{v}$ for different background variables. Information that is important for prediction is captured in $\mathbf{v}$, so we can visualize the important factors by the separation in the components of $\mathbf{v}$. We see sex,.,and  are important variables, because of their separation.

% Not done yet...
%\subsection{Bootstrapping and cross-validation}

%A held-out portion of the data containing 20\% of the individuals is used as the test set. The remaining 80\% of the data is used for the training and validation sets. The training and validation sets are selected by 5-fold cross-validation on this remaining portion of the data. 

%To evaluate the robustness of the inferred network, we bootstrap each of the training sets in this cross-validation 25 times. Bootstrapped 95\% confidence intervals are computed with quantiles of the bootstrap distribution, $\mathrm{CI} = (q_{0.25}, q_{0.975})$.

%To calculate the full likelihood, we would need to compute the expectation of this conditional likelihood over all trajectories,
%\begin{eqnarray}
%\log{p(Y^{(m)}, a^{(m)};\theta)} =\mathbb{E}_{\mathcal{T}}\Big[\log{p(Y^{(m)}|\mathcal{T},\theta)}\Big],
%\end{eqnarray}
%where the trajectories are sampled from Equations \ref{dynamics} and \ref{survival} given the initial baseline at $t_0$.

%However, simply maximizing this likelihood can result in over-fitting the diffusive trajectory noise $\sigma_x$ to zero. This occurs because stochastic deviations from the maximum likelihood fit of the trajectories lowers the likelihood, which will force $\sigma_x\to 0$


%To forecast the future health trajectory and survival of an individual, we only use their baseline data at age $t_0$. One reason for this is that in the ELSA dataset, there are only 8 waves of measurements, and so taking multiple as input restricts the amount of data available for training. Additionally, our SDE approach is much simpler with only an initial state at $t_0$.
%Want to add this but still need to think about it a bit. There are different ways in which using multiple input times can come in, e.g. just using it for better imputation or using a conditioned diffusion process (Ryder:2018). 


may not work well, because we expect that the , and so we would like these to be as accurate as possible.

%Additionally, values that are observed are noisy and cannot be reliably be taken as the initial values.  (Questionable)
%``Will not work'' is a very strong statement. We should either show this (and emphasize more) or tone this down to ``do not work as well''

%Auto-encoders have been used for ``denoising'' and ``inpainting'', where they can remove noise or fill in missing regions on an image (\cite{Xie:2012}). Our application is similar, we want to estimate the missing variables at the initial time point and also remove noise from the observed values that we do have. (\cite{Goodfellow:2016}

%
%
%\begin{eqnarray} \label{autoencoder}
%\mathbf{x}(t_0) &=& f(\mathbf{y}_{t_0} +\epsilon_y, \mathbf{m}_{t_0}, t_0, \mathbf{u}), 
%\end{eqnarray}
%
%where $f$ is a non-linear function represented as a neural network that uses the observed values, missing mask, age, and static variables as input to predict the missing values. 


%We compute the likelihood in the standard way for joint longitudinal-survival models, $\log{p(Y, T;\theta)} = \log{p(Y;\theta)} + \log{p(T|Y;\theta)}$. 


%
%\begin{eqnarray} \label{corruption}
%\tilde{\mathbf{o}}_{t_0} &=& %\mathbf{c}\odot\mathbf{o}_{t_0},\,\,\mathbf{c}\sim\mathrm{Bernoulli}(p_c), \\ \nonumber
%\tilde{\mathbf{y}}_{t_0} &=& \tilde{\mathbf{o}}_{t_0}\odot(\mathbf{y}_{t_0} + \epsilon_y) + (1 - \tilde{\mathbf{o}}_{t_0})\odot\mathbf{\epsilon},\,\,\mathbf{\epsilon}\sim\mathcal{N}(0,\mathbf{I}), \nonumber
%\end{eqnarray}



%Our implementation of survival in the model resembles joint longitudinal survival models \cite{Yashin:2007, Lim:2018}.
%add here/fix
% currently this section is sparse (in terms of text). Maybe worth a structure for each figure: 
% what do we want to assess, why is this measure the good way of doing it, how is it measured in detail, how is the figure presented, what do we observe or what questions arise about the data shown
% I think of the discussion at the end as discussion of the figures/results/method together (broader questions) rather than 
% discussion of the figure details. I think those figure details can be in the results (subject to objection by referees) and can help people digest the figure -- as they try to see what we describe seeing.
%


% it is worth considering a more plot driven approach. Right now you go with shock-and-awe, going straight to the model behavior. Fig 2-4.
% you might rather build the model up (so start with the latent space and missing variables, including quantitative validation) and only at the very end show the longitudinal trajectories. 
% this may have the advantage of letting readers/referees understand how it is built, but also appreciating those building blocks for themselves. It may also facilitate a more coherent discussion of the results as we go (and so better understanding by reader)
% This sort of large rearrangement is much easier at this point, but not so difficult at any stage.

